Time-to-reach Bounds for Verification of Dynamical Systems Using the Koopman Spectrum

In this work, we present a novel Koopman spectrum-based reachability verification method for nonlinear systems. Contrary to conventional methods that focus on characterizing all potential states of a dynamical system over a presupposed time span, our approach seeks to verify the reachability by assessing the non-emptiness of estimated time-to-reach intervals without engaging in the explicit computation of reachable set. Based on the spectral analysis of the Koopman operator, we reformulate the problem of verifying existence of reachable trajectories into the problem of determining feasible time-to-reach bounds required for system reachability. By solving linear programming (LP) problems, our algorithm can effectively estimate all potential time intervals during which a dynamical system can enter (and exit) target sets from given initial sets over an unbounded time horizon. Finally, we demonstrate our method in challenging settings, such as verifying the reachability between non-convex or even disconnected sets, as well as backward reachability and multiple entries into target sets. Additionally, we validate its applicability in addressing real-world challenges and scalability to high-dimensional systems through case studies in verifying the reachability of the cart-pole and multi-agent consensus systems.

==> related_work.tex <==
\section{Related work}

% \color{blue}
% \begin{itemize}
%     \item Focus specifically on Koopman-based reachability and verification such as \cite{umathe2022reachability} and \cite{bak2022reachability}.
% \end{itemize}

Given that linear dynamical systems permit closed-form solutions along with a wide array of techniques for their analysis, prediction, and control, the extension of these methodologies to nonlinear systems through the construction of linear approximations has been a prevailing research focus within the control community. 
% This approach facilitates the transposition of techniques from linear systems to tackle issues related to nonlinear systems, thereby broadening the scope of existing methodologies to handle intricate nonlinear dynamics.

Unlike local linear approximation techniques such as Taylor series expansion, by representing a nonlinear dynamical systems in terms of an infinite-dimensional operator acting on a Hilbert space of measurement functions of the system state, Koopman operator theory \cite{koopman1931hamiltonian} has garnered significant attention in control research due to its ability to achieve global linearization of nonlinear systems.
% By representing a nonlinear dynamical systems in terms of an infinite-dimensional operator acting on a Hilbert space of measurement functions of the system state, numerous techniques for prediction and control in linear systems have been extended to address nonlinear systems, including reachability analysis.
While the Koopman operator is theoretically defined as an infinite-dimensional linear operator, it can be approximated in a finite-dimensional form using techniques like Dynamic Mode Decomposition (DMD) and its various extensions \cite{schmid2022dynamic} and Krylov-subspace methods \cite{mezic2022numerical}.

Additionally, considering the critical role of Koopman spectral theory in facilitating the analysis and control of dynamical system, innovative methods such as the path-integral method \cite{deka2023path} and Laplace average method \cite{mauroy2013isostables}\cite{deka2023supervised} have been developed recently to numerically evaluate the principal eigenfunctions over specific domains, and its combination with neural networks \cite{deka2022koopman} has further enhanced flexibility in approximating eigenfunctions, thus providing a more practical framework for the study of dynamical systems.

Naturally, such a Koopman-based perspective of dynamical systems has led to the development of various methodologies for Koopman theory-based reachability analysis.
% There are two primary streams within Koopman theory-based reachability analysis methods.
% Reachability analysis methods based on Koopman theory can be generally categorized into two categories.
One of the first algorithms in this direction was proposed in \cite{bak2021reachability}, where the authors verify the reachability of black-box nonlinear systems with Koopman linearization and zonotope over-approximations of nonlinear initial sets.
Subsequently, \cite{bak2022reachability} advance this idea by employing random Fourier features to improve the accuracy of linearization, and combining Taylor models with polynomial zonotope refinement to handle the nonlinear transformation of the initial states.
The reachability of the Koopman bilinear form of control-affine nonlinear systems is discussed in \cite{goswami2021bilinearization}.
In contrast, other methods seek to utilize the Koopman spectrum to analyze the reachability of the system. The authors in \cite{umathe2022reachability} use the principal eigenfunctions of the Koopman operator for the characterization of both forward and backward reachable sets, and provide formal guarantees for the set approximation under the Hausdorff metric. %Application for approximating reachable sets for vehicle dynamics with the principle eigenfunctions is detailed in \cite{kumar2023reachability}.

% data-driven techniques like Extended Dynamic Mode Decomposition (EDMD) \cite{williams2015data} enable finite dimensional approximations of it.




